Positive Unlabeled Contrastive Learning

Self-supervised pretraining on unlabeled data followed by supervised fine-tuning on labeled data is a popular paradigm for learning from limited labeled examples. We extend this paradigm to the classical positive unlabeled (PU) setting, where the task is to learn a binary classifier given only a few labeled positive samples, and (often) a large amount of unlabeled samples (which could be positive or negative). We first propose a simple extension of standard infoNCE family of contrastive losses, to the PU setting; and show that this learns superior representations, as compared to existing unsupervised and supervised approaches. We then develop a simple methodology to pseudo-label the unlabeled samples using a new PU-specific clustering scheme; these pseudo-labels can then be used to train the final (positive vs. negative) classifier. Our method handily outperforms state-of-the-art PU methods over several standard PU benchmark datasets, while not requiring a-priori knowledge of any class prior (which is a common assumption in other PU methods). We also provide a simple theoretical analysis that motivates our methods.

==> Notes/convergence.tex <==
~\cite{moulines2011non, needell2014stochastic, needell2016batched} 

==> Notes/defpack.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{algorithm}
\usepackage{algorithmic}
% \newcommand{\theHalgorithm}{\arabic{algorithm}}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}
\usepackage{comment}
\usepackage{bm}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[]{Lemma}
\newtheorem{proposition}{Proposition}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}[]
\newtheorem{assumption}{Assumption}[]
\newtheorem{fact}{Fact}[]
%\theoremstyle{remark}
\newtheorem{remark}{Remark}[]

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\renewcommand{\qedsymbol}{$\blacksquare$}

% % Figure reference, lower-case.
% \def\figref#1{figure~\ref{#1}}
% % Figure reference, capital. For start of sentence
% \def\Figref#1{Figure~\ref{#1}}
% \def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
% \def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% % Section reference, lower-case.
% \def\secref#1{section~\ref{#1}}
% % Section reference, capital.
% \def\Secref#1{Section~\ref{#1}}
% % Reference to two sections.
% \def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% % Reference to three sections.
% \def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% % Reference to an equation, lower-case.
% \def\eqref#1{equation~\ref{#1}}
% % Reference to an equation, upper case
% \def\Eqref#1{Equation~\ref{#1}}
% % A raw reference to an equation---avoid using if possible
% \def\plaineqref#1{\ref{#1}}
% % Reference to a chapter, lower-case.
% \def\chapref#1{chapter~\ref{#1}}
% % Reference to an equation, upper case.
% \def\Chapref#1{Chapter~\ref{#1}}
% % Reference to a range of chapters
% \def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% % Reference to an algorithm, lower-case.
% \def\algref#1{algorithm~\ref{#1}}
% % Reference to an algorithm, upper case.
% \def\Algref#1{Algorithm~\ref{#1}}
% \def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
% \def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% % Reference to a part, lower case
% \def\partref#1{part~\ref{#1}}
% % Reference to a part, upper case
% \def\Partref#1{Part~\ref{#1}}
% \def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\mathbf{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\mathbf{0}}}
\def\vone{{\mathbf{1}}}
\def\vmu{{\mathbf{\mu}}}
\def\vtheta{{\mathbf{\theta}}}
\def\va{{\mathbf{a}}}
\def\vb{{\mathbf{b}}}
\def\vc{{\mathbf{c}}}
\def\vd{{\mathbf{d}}}
\def\ve{{\mathbf{e}}}
\def\vf{{\mathbf{f}}}
\def\vg{{\mathbf{g}}}
\def\vh{{\mathbf{h}}}
\def\vi{{\mathbf{i}}}
\def\vj{{\mathbf{j}}}
\def\vk{{\mathbf{k}}}
\def\vl{{\mathbf{l}}}
\def\vm{{\mathbf{m}}}
\def\vn{{\mathbf{n}}}
\def\vo{{\mathbf{o}}}
\def\vp{{\mathbf{p}}}
\def\vq{{\mathbf{q}}}
\def\vr{{\mathbf{r}}}
\def\vs{{\mathbf{s}}}
\def\vt{{\mathbf{t}}}
\def\vu{{\mathbf{u}}}
\def\vv{{\mathbf{v}}}
\def\vw{{\mathbf{w}}}
\def\vx{{\mathbf{x}}}
\def\vy{{\mathbf{y}}}
\def\vz{{\mathbf{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\mathbf{A}}}
\def\mB{{\mathbf{B}}}
\def\mC{{\mathbf{C}}}
\def\mD{{\mathbf{D}}}
\def\mE{{\mathbf{E}}}
\def\mF{{\mathbf{F}}}
\def\mG{{\mathbf{G}}}
\def\mH{{\mathbf{H}}}
\def\mI{{\mathbf{I}}}
\def\mJ{{\mathbf{J}}}
\def\mK{{\mathbf{K}}}
\def\mL{{\mathbf{L}}}
\def\mM{{\mathbf{M}}}
\def\mN{{\mathbf{N}}}
\def\mO{{\mathbf{O}}}
\def\mP{{\mathbf{P}}}
\def\mQ{{\mathbf{Q}}}
\def\mR{{\mathbf{R}}}
\def\mS{{\mathbf{S}}}
\def\mT{{\mathbf{T}}}
\def\mU{{\mathbf{U}}}
\def\mV{{\mathbf{V}}}
\def\mW{{\mathbf{W}}}
\def\mX{{\mathbf{X}}}
\def\mY{{\mathbf{Y}}}
\def\mZ{{\mathbf{Z}}}
\def\mBeta{{\mathbf{\beta}}}
\def\mPhi{{\mathbf{\Phi}}}
\def\mLambda{{\mathbf{\Lambda}}}
\def\mSigma{{\mathbf{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\mathbf{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \mathbf wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution
\newcommand{\ts}{\textsuperscript}

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Notes/exp.tex <==
Please check the \href{https://github.com/anishacharya/SGD_PU/blob/main/synthetic.ipynb}{Jupyter Notebook} for experiments on synthetic data. 

\paragraph{\bf Datasets.} In this setting we take the usual MNIST, CIFAR10 datasets and treat samples with odd labels as positive and even labels as negative. In order to construct PU dataset from Binary MNIST / CIFAR10 we assume that the true target $y \in \{ 0, 1\}$ is unavailable during training and instead another random variable $s \in \{0, 1\}$ is noted where $s=1$ means labeled and $s=0$ denote unlabeled samples and thus our training data is of the form $\gD_t = \{ (\vx_1, s_1), \dots , (\vx_n, s_n)\}$ where all the labeled data is positive i.e. $P(y=1 | s=1) = 1$. For our experiments we assume $k$ of the $n$ samples are labeled positive i.e. $s=1$ and rest $n-k$ samples are unlabeled i.e. $s=0$. Noting that for MNIST and CIFAR10 we have roughly 30k samples belonging to true positive and true negative classes we repeat our PU experiment with $k= 3k, 10k, 15k, 20k, 25k$ respectively.    

\paragraph{\bf PN Baselines:} A naive approach is to essentially treat all the unlabeled samples as negative samples and train a traditional binary \underline{P}ositive \underline{N}egative (PN) classifier. We will refer to this approach as {\bf \textsc{NaivePU}}. For a moment let us assume \textsc{Naive-PU} works. One immediate improvement can be to introduce some loss re-weighting mechanism to mitigate the bias introduced by the class imbalance as number of unlabeled samples (treated as negative by \textsc{Naive-PU}) is much larger than number of positive samples. The most widely adopted approach is to re-weight the samples using inverse class frequency or a smoothed inverse square root of class frequency~\citep{cui2019class, wang2017learning, huang2016learning}. We simply create a baseline by re-weighting the samples by inverse class frequency and refer to this as Class Balanced \textsc{NaivePU} abbreviated as {\bf \textsc{CB-NaivePU}}. 

\begin{table}[]
\centering
\begin{tabular}{@{}llllll@{}}
\toprule
                 & Vanilla & uPU   & Self PU & SSL + FT & SSL + init \\ \midrule
Supervised       & {\bf 98.96}   & 98.87 & 98.04       & 95.64   & 98.95     \\
P (3k) , U (57k) & 50.72   & 93.88 & 96      & 95.46   & {\bf 97.05}     \\
P (1k) , U (59k) & 50.72   & 92.52 & 94.21   & 94.18   & {\bf 96.77}     \\ \bottomrule
\end{tabular}
\caption{}
\label{tab:bin_mnist.results}
\end{table}

==> Notes/explain.tex <==
\subsection{Gradient Diversity}
\cite{ash2019deep} computes gradients with respect to the last layer and samples a batch of examples where the gradients span a diverse set of directions \textcolor{red}{Explaining PC Pursuit ?} for continual learning. ~\cite{yin2018gradient}
\paragraph{Notation} Batch Size: $B$, Number of clients: $P$, $\frac{B}{P}$ samples per client node, Total number of points $n$ implying $\frac{n}{B}$ iterations per epoch.  

\paragraph{Optimal Scaling}  \textcolor{red}{Do Literature survey on what is the best known bound for optimal scaling}. If we increase $P$ we don't see optimal speedup. \textbf{speedup saturation}. One cause can be communication bottleneck. 

\subsection{Model Uncertainty}
\cite{ash2019deep} apply use model uncertainty for continual learning. They measures model uncertainty as the magnitude (we can do norm) of the gradient with respect to the last layer.

\subsection{Active Learning}




==> Notes/intro.tex <==
Consider optimization problems with finite sum structure: 
\begin{equation}
    \label{equation:finite_sum}
    \min_{\vw \in \R^d} \left[\bar{f}({\vw}):=\frac{1}{n}\sum_{i=1}^n f_i(\vw)\right].
\end{equation}
Note that, this formulation is typical in modern ML algorithms solved under Empirical Risk Minimization (ERM) framework, where $f_i(\vw)$ corresponds to the loss of a model with parameters $\vw \in \sR^d$ on training example $i$ from the training dataset of size
$n$ and $\bar{f}({\vw})$ represents the empirical risk. Mini-batch SGD is the de-facto method for optimizing such functions \cite{robbins1951stochastic, bottou2010large, tsitsiklis1986distributed} which proceeds as follows: \\
At each iteration $t$, it selects a random batch $\gD_t$ of $b$ samples, obtains gradients $\vg_t^{(i)}=\nabla f_i(\vw_t), \;\forall i \in \gD_t$, and updates the parameters using iterations of the form: 
\begin{equation}
\label{equation:sgd}
\vw_{t+1} := \vw_t - \gamma \tilde{\vg}_t ,\quad 
\tilde{\vg}_t = \frac{1}{|\gD_t|} \sum_{i\in \gD_t} \vg_t^{(i)}.
\end{equation}
In this monograph we are interested in analyzing first order gradient based methods like SGD under the \underline{P}ositive \underline{U}nlabeled (PU) setting where only a small fraction of positive data is available along with a large amount of unlabeled data.  



==> Notes/our_approach.tex <==
Our approach treats the PU Learning problem as a self supervised learning (SSL) problem. Our idea is to train a model using contrastive loss over all the training data (both P and U), and then fine-tune a linear head on top of the learned representation to learn a final model. This approach has been widely successful in leveraging SSL in downstream tasks like image classification. However, one issue with this approach is that in the PU setting we do not have samples from all the classes to finetune on. To alleviate this we propose a two step process which proceeds as follows: 
\\
(a) PreTrain over all available data (P and U) using contrastive loss to learn good representation. 
\\
(a) Identify confident positive and negative samples in an iterative fashion to create a trusted set.
\\
(b) Freeze the representation; attach and Fine-tune online head using the trusted set. 

\subsection{Contrastive PreTraining}
\subsection{Trusted Set}
The key step in our approach is to identify 

\subsection{}


==> Notes/related.tex <==
Dating back to the works of~\cite{denis1998pac} PU Learning refers to the \textbf{weakly supervised} task of learning a binary classifier without any explicitly labeled negative examples i.e. using only positive and unlabeled samples. Further, in most practical settings the data is highly imbalanced meaning the learner has access to only a small number of positive labeled data and a large pool of unlabeled data. As a running example, consider the problem of personalized recommendation: \textcolor{red}{(example applications)}. Owing to the importance of the problem in several real world problems and recent advances in semi supervised learning, developing specialized learning algorithms for PU setting have received renewed impetus in the machine learning community. Most of the recent research in this area can be broadly categorized into the following categories: 

\subsection{Cost Sensitive Learning Approach}
Recall that PU dataset, sampled uniformly at random (u.a.r) from an underlying distribution $P(\rx, \ry)$ is composed of a set of samples with positive class $\sX_{+}$ and a set of 
unlabeled samples $\sX_{u}$. Following the formulations in ~\citep{elkan2008learning, du2014analysis, christoffel2016class}, we note that unlabeled data can be treated as a mixture of both positive and negative samples.  
\begin{align}
    \sX_{+} = \{\vx_{i}\}_{i=1}^{n_0} \sim p(\rx | \ry = 1), \; \sX_{u} = \{\vx_{i}\}_{i=n_0 + 1}^{n} \sim p(\rx); \; \sX = \sX_{+} \cup \sX_{u}
\end{align}
Letting $\pi_+ = p(y=1)$ to be the class prior we can write the marginal density as: 
\begin{flalign}
\label{equation:unlabeled_distribution}
    p(\vx) = \pi_+ p(\vx | y=1) + (1- \pi_+) p(\vx | y = 0)
\end{flalign}
Note that the goal is to learn a model $g_\vw(\vx)$ parameterized by $\vw$ such that: $g_\vw(\vx) \approx p(y=1|\vx)$.
However, we don't have information about $y$. Hence it is convenient to define another random variable $s$ as:
\begin{flalign}
s = 
\begin{cases}
1 \; &\text{if } \vx \text{ is labeled}\\
0 \; &\text{o/w}
\end{cases}
\end{flalign}
Now viewing $\vx, y, s$ as random variables allows us to assume that there is some true underlying distribution $p(\vx, y, s)$ over triplets $(\vx, y, s)$. $\sX$ is sampled from $p(\vx, y, s)$ however, for each sampled triplet only $(\vx, s)$ is recorded.
This also implies that when $s = 1$ then $y=1$ is certain.
\begin{flalign}
& P(y = 1 | \vx, s = 1) = P(y = 1 | s = 1) = 1
\end{flalign}
Additionally, recall that in the PU setting only the positive data can be labeled i.e. formally: 
\begin{flalign}
p(s=1 | \vx, y=0) = p(s=1 | y=0) = 0 
\end{flalign}
If we train a classifier $g'_{\vw'}(\vx)$ on the positive: $s=1$ , unlabeled: $s=0$, it will yield $g'_{\vw'}(\vx) \approx p(s=1 | \vx)$. The main goal would be to estimate $g_\vw(\vx)$ from the surrogate $g'_{\vw'}(\vx)$. It is clear that, without some assumption about which positive samples are labeled, learning is impossible. 
\begin{assumption}[{\bf SCAR : Selected Completely At Random}]
\label{assm:selected_at_rand}
The labeled positive samples are sampled uniformly at random from all positive examples~\citep{elkan2008learning}. Formally speaking:
\begin{flalign}
p(s=1 | \vx, y=1) = p(s=1 | y=1) = c
\end{flalign}
Intuitively, this simply means if the true label $y=1$ then the probability that a positive sample is labeled is {\bf constant} regardless of $\vx$ i.e. {\bf $s$ and $\vx$ are conditionally independent given $y$}. In other words it means that {\bf all the positive examples have the same probability of being labeled}. Note that SCAR is equivalent to the missing completely at random assumption commonly made for learning from data with missing values~\citep{liu2003building, smith2007making}.
\end{assumption}
\begin{lemma}[~\cite{elkan2008learning}]
\label{lemma:surrogate}
If Assumption~\ref{assm:selected_at_rand} holds, then $p(y = 1 | \vx) = p(s = 1 | \vx) / c$ where the constant is given by $c = p(s = 1 | y = 1 )$
\end{lemma}
\begin{proof}
\begin{flalign*}
p(s=1|\vx) &= p(y=1 \wedge s = 1 | \vx)\\ 
&= p(s=1| y=1,\vx) \cdot p(y=1 | \vx)\\
&= c \cdot p(y=1 | \vx) \;\; \text{(using Assumption~\ref{assm:selected_at_rand})}
\end{flalign*}
The proof is complete by diving both side by $c$.
\end{proof}

\begin{remark}
If Assumption~\ref{assm:selected_at_rand} holds, $0 \leq p(s = 1 | \vx) \leq p(s=1|y=1)$ 
\end{remark}
\begin{proof}
Since $p(y=1|\vx)$ is a well defined probability measure thus we have:
$0 \leq p(y=1|\vx) \leq 1$ , thus using Lemma~\ref{lemma:surrogate} we immediately get the desired result by multiplying both side by $c$. \footnote{Another way of thinking about this problem is through the fact that positive and negative(unlabeled) training sets for the surrogate are from overlapping region in the probability space. Let $n$ be total number of samples, $n_l$ are labeled and $n_u$ unlabeled i.e. $n = n_l + n_u$. Further suppose that number of true positive samples are $n_+$ and number of true negatives $n_-$ and $n = n_+ + n_-$. Thus, we have $p(s=1 | y=1) = \frac{n_l}{n_+}
\geq \frac{n_l}{n}
= p(s=1 | \vx)$
Since the other side of the inequality is trivial, this concludes the proof.
}
\end{proof}

% However, in many real world scenarios the SCAR assumption might not be practical due to biases in observed positive labels~\citep{bekker2019beyond, su2021positive}. To deal with this some works also consider the following more relaxed assumptions.

% \begin{assumption}[\bf SAR: Selected At Random]

% \end{assumption}

% \begin{assumption}[\bf SNAR: Selected Not At Random]

% \end{assumption}

% \paragraph{Class Prior Estimation.}
% If the class prior $\pi$ of the unlabeled dataset is known, then the PU Learning problem~\eqref{equation:unlabeled_distribution} can be reduced to cost-sensitive learning~\citep{elkan2001foundations} over positive and unlabeled data. Let $\mC$ be the cost matrix then $\mC[i,j]$ i.e. the $(i,j)$ th entry denote the cost of predicting class $i$ when true class is $j$. 

\subsection{Two-step Techniques}
At a high level these approaches use some heuristic to identify potential (with high confidence) negative samples from the unlabeled pool of data; then together with the positive data learn a traditional supervised learner ~\citep{luo2021pulns, bekker2020learning}. Some works instead identify potential positives from the unlabeled samples and augments to the existing P samples. More recently,~\citep{chen2020self} combined the two ideas and instead identifies both positive and negative samples from the unlabeled set. 




==> Notes/uPU.tex <==
Let $\rx \in \sR^d$, $d \in \sN$ , $\ry \in \{\pm 1\}$ be the input and output random variables and $p(\rx, \ry)$ be the underlying joint distribution of $(\rx, \ry)$. 
A PU dataset $\gX$, sampled uniformly at random from $p(\rx, \ry)$ is composed of an incomplete set $\gX_{P}$ of $n_p$ samples with positive class and a set $\gX_{U}$ of $n_u$ unlabeled samples. Without loss of generality, it can be assumed that $\gX_P$ and $\gX_U$ are sampled independently from the P marginal and U marginal respectively~\citep{kiryo2017positive}.
\begin{equation}
\label{eq:pu_dataset}
    \gX_P = \{\vx_i^P\}_{i=1}^{n_p} \sim p(\rx | \ry = 1);\; \gX_U = \{\vx_i^U\}_{i=1}^{n_u} \sim p(\rx);\; \gX = \gX_P \cup \gX_U
\end{equation}



==> assets/algo/algo.ConPU.tex <==

% Denote the P marginal as $p_p(\rx) = p(\rx | \ry=1)$, N marginal $p_n(\rx) = p(\rx | \ry=-1)$ and U marginal $p(\rx)$; let $\ell:\sR\times\{\pm 1\}\to \sR$ be the loss function i.e. $\ell(g(\rx), \ry)$ is the loss incurred by $\net$ on sample $\rx$ when the ground truth is $\ry$. 
% If class prior probability $\pi=p(\ry=1)$ is known, then under the empirical risk minimization (ERM) framework the empirical risk is: $R(g)= \pi R_p^+(g)+(1-\pi)R_n^-(g)$. In the fully supervised setting expected positive and negative risks can be directly estimated from the training data as:
% $R_p^+(g) = \E_{\rx \sim p_p}[\ell(\net(\rx),+1)] = \frac{1}{n_p}\sum_{i=1}^{n_p}\ell(\net(\rx_i^P), +1)$ and $R_n^-(g) = \E_{\rx \sim p_n}[\ell(\net(\rx),-1)] = \frac{1}{n_n}\sum_{i=1}^{n_n}\ell(\net(\rx_i^N),-1)$.
% % $R_p^+(g) = \frac{1}{n_p}\E_{\rx \sim p_p}[\ell(\net(\rx), +1)]$ and $R_n^-(g) = \frac{1}{n_n}\E_{\rx \sim p_n}[\ell(\net(\rx), -1)]$.


% \subsection{Cost Sensitive Learning Approach}
% Recall that PU dataset, sampled uniformly at random (u.a.r) from an underlying distribution $P(\rx, \ry)$ is composed of a set of samples with positive class $\sX_{+}$ and a set of 
% unlabeled samples $\sX_{u}$. Following the formulations in ~\citep{elkan2008learning, du2014analysis, christoffel2016class}, we note that unlabeled data can be treated as a mixture of both positive and negative samples.  
% \begin{flalign}
%     \sX_{+} 
%     &= \{\vx_{i}\}_{i=1}^{n_0} \sim p(\rx | \ry = 1)\\
%     \sX_{u}
%     &= \{\vx_{i}\}_{i=n_0 + 1}^{n} \sim p(\rx)\\
%     \sX &= \sX_{+} \cup \sX_{u}
% \end{flalign}
% Letting $\pi_+ = p(y=1)$ to be the class prior we can write the marginal density as: 
% \begin{flalign}
% \label{equation:unlabeled_distribution}
%     p(\vx) = \pi_+ p(\vx | y=1) + (1- \pi_+) p(\vx | y = 0)
% \end{flalign}
% Note that the goal is to learn a model $g_\vw(\vx)$ parameterized by $\vw$ such that: $g_\vw(\vx) \approx p(y=1|\vx)$.
% However, we don't have information about $y$. Hence it is convenient to define another random variable $s$ as:
% \begin{flalign}
% s = 
% \begin{cases}
% 1 \; &\text{if } \vx \text{ is labeled}\\
% 0 \; &\text{o/w}
% \end{cases}
% \end{flalign}
% Now viewing $\vx, y, s$ as random variables allows us to assume that there is some true underlying distribution $p(\vx, y, s)$ over triplets $(\vx, y, s)$. $\sX$ is sampled from $p(\vx, y, s)$ however, for each sampled triplet only $(\vx, s)$ is recorded.
% This also implies that when $s = 1$ then $y=1$ is certain.
% \begin{flalign}
% & P(y = 1 | \vx, s = 1) = P(y = 1 | s = 1) = 1
% \end{flalign}
% Additionally, recall that in the PU setting only the positive data can be labeled i.e. formally: 
% \begin{flalign}
% p(s=1 | \vx, y=0) = p(s=1 | y=0) = 0 
% \end{flalign}
% If we train a classifier $g'_{\vw'}(\vx)$ on the positive: $s=1$ , unlabeled: $s=0$, it will yield $g'_{\vw'}(\vx) \approx p(s=1 | \vx)$. The main goal would be to estimate $g_\vw(\vx)$ from the surrogate $g'_{\vw'}(\vx)$. It is clear that, without some assumption about which positive samples are labeled, learning is impossible. 

% \begin{lemma}[~\cite{elkan2008learning}]
% \label{lemma:surrogate}
% If Assumption~\ref{assm:selected_at_rand} holds, then $p(y = 1 | \vx) = p(s = 1 | \vx) / c$ where the constant is given by $c = p(s = 1 | y = 1 )$
% \end{lemma}
% \begin{proof}
% \begin{flalign*}
% p(s=1|\vx) &= p(y=1 \wedge s = 1 | \vx)\\ 
% &= p(s=1| y=1,\vx) \cdot p(y=1 | \vx)\\
% &= c \cdot p(y=1 | \vx) \;\; \text{(using Assumption~\ref{assm:selected_at_rand})}
% \end{flalign*}
% The proof is complete by diving both side by $c$.
% \end{proof}

% \begin{remark}
% If Assumption~\ref{assm:selected_at_rand} holds, $0 \leq p(s = 1 | \vx) \leq p(s=1|y=1)$ 
% \end{remark}
% \begin{proof}
% Since $p(y=1|\vx)$ is a well defined probability measure thus we have:
% $0 \leq p(y=1|\vx) \leq 1$ , thus using Lemma~\ref{lemma:surrogate} we immediately get the desired result by multiplying both side by $c$. \footnote{Another way of thinking about this problem is through the fact that positive and negative(unlabeled) training sets for the surrogate are from overlapping region in the probability space. Let $n$ be total number of samples, $n_l$ are labeled and $n_u$ unlabeled i.e. $n = n_l + n_u$. Further suppose that number of true positive samples are $n_+$ and number of true negatives $n_-$ and $n = n_+ + n_-$. Thus, we have $p(s=1 | y=1) = \frac{n_l}{n_+}
% \geq \frac{n_l}{n}
% = p(s=1 | \vx)$
% Since the other side of the inequality is trivial, this concludes the proof.
% }
% \end{proof}

==> assets/algo/ass.scar.tex <==
\begin{assumption}[{\bf SCAR : Selected Completely At Random}]
\label{assm:selected_at_rand}
The labeled positive samples are sampled uniformly at random from all positive examples~\citep{elkan2008learning}. Formally speaking:
\begin{flalign}
p(s=1 | \vx, y=1) = p(s=1 | y=1) = c
\end{flalign}
Intuitively, this simply means if the true label $y=1$ then the probability that a positive sample is labeled is {\bf constant} regardless of $\vx$ i.e. {\bf $s$ and $\vx$ are conditionally independent given $y$}. In other words it means that {\bf all the positive examples have the same probability of being labeled}. Note that SCAR is equivalent to the missing completely at random assumption commonly made for learning from data with missing values~\citep{liu2003building, smith2007making}.
\end{assumption}

==> assets/algo/tab.losses.tex <==
\begin{table*}[]
\small
\caption{}
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
Loss & Label & Empirical Risk
\\ 
\midrule
\midrule
infoNCE~\citep{chen2020simple} 
& \textcolor{red}{\xmark}
&
$\ell_{infoNCE}^{(i)}=-\log \frac{\exp{(\vz_i^{t}} \boldsymbol \cdot \vz_{j(i)}^{t}/\tau)}{\sum_{k \in \sI \setminus \{i\}} \exp{(\vz_i^t \boldsymbol \cdot \vz_k^t / \tau)}}, \forall i \in \sI$
\\
DCL~\citep{chuang2020debiased}
& \textcolor{red}{\xmark}
& 
$-\sum_{i \in \sI} \left[\log \frac{
\exp{(\vz_i^{t}} 
\boldsymbol \cdot \vz_{j(i)}^{t}/\tau)}
{\exp{(\vz_i^{t}} 
\boldsymbol \cdot \vz_{j(i)}^{t}/\tau)
+
\sum_{k \in \sI \setminus \{i\}} \exp{(\vz_i^t \boldsymbol \cdot \vz_k^t / \tau)}}\right]$
\\
suNCEt~\citep{assran2020supervision} 
& \textcolor{green}{\cmark}
& $\ell^{(i)}_{suNCEt} = 
\begin{cases}
-\log \frac{\sum_{j\in \sP \setminus \{i\}}\exp{(\vz_i^{t}} \boldsymbol \cdot \vz_j^t/\tau)}{\sum_{k \in \sI \setminus \{i\}} \exp{(\vz_i^t \boldsymbol \cdot \vz_k^t / \tau)}}, \forall i\in \sP\\
\ell_{infoNCE}^{(i)}, \forall i \in \sI \setminus \sP
\end{cases}
$             
\\
supCon~\citep{khosla2020supervised} 
& \textcolor{green}{\cmark}
& $\ell^{(i)}_{supCon} = 
\begin{cases}
-\frac{1}{|\sP|-1}\sum_{j\in \sP \setminus \{i\}}\log \frac{\exp{(\vz_i^{t}} \boldsymbol \cdot \vz_j^t/\tau)}{\sum_{k \in \sI \setminus \{i\}} \exp{(\vz_i^t \boldsymbol \cdot \vz_k^t / \tau)}}, \forall i\in \sP\\
\ell_{infoNCE}^{(i)}, \forall i \in \sI \setminus \sP
\end{cases}
$             
\\
puNCE {\bf (This Work.)}  
& \textcolor{green}{\cmark}
& $\ell^{(i)}_{puNCE} = 
\begin{cases}
-\frac{1}{|\sP|-1}\sum_{j\in \sP \setminus \{i\}}\log \frac{\exp{(\vz_i^{t}} \boldsymbol \cdot \vz_j^t/\tau)}{\sum_{k \in \sI \setminus \{i\}} \exp{(\vz_i^t \boldsymbol \cdot \vz_k^t / \tau)}}, \forall i\in \sP\\

   -\frac{\pi}{|\sP|-1}\sum_{j\in \sP \setminus \{i\}}\log \frac{\exp{(\vz_i^{t}} \boldsymbol \cdot \vz_j^t/\tau)}{\sum_{k \in \sI \setminus \{i\}} \exp{(\vz_i^t \boldsymbol \cdot \vz_k^t / \tau)}}\\ 
- (1 - \pi)\ell_{infoNCE}^{(i)} \;,
\forall i \in \sI \setminus \sP 
\end{cases}
$
\\
\bottomrule
\end{tabular}

\label{tab:loss_equation}
\end{table*}

==> assets/algo/theory.tex <==
Suppose we are given a PU dataset~\eqref{eq:pu_dataset} and the class prior probability $\pi=p(\ry=1)$. Let $\net: \sR^d \to \sR$ be the decision function at iteration $t$ and $\ell:\sR\times\{\pm 1\}\to \sR$ is the loss function. This implies that $\ell(g(\rx), \ry)$ is the loss incurred by $\net$ on sample $\rx$ when the ground truth is $\ry$. For notational convenience, let us denote the P marginal as $p_p(\rx) = p(\rx | \ry=1)$, N marginal $p_n(\rx) = p(\rx | \ry=-1)$ and U marginal $p(\rx)$. In the standard fully supervised learning setting (referred to as Positive Negative (PN) learning hereafter), since negative labels are available, we can write the risk as: 
\begin{flalign}
    R(g) &= \pi R_p^+(g) + (1- \pi)R_n^-(g)
\label{eq:risk.def}
\end{flalign}
Where $R_p^+(g)$ and $R_n^-(g)$ are positive and negative risks respectively and are defined as:
\begin{flalign}
R_p^+(g) = \E_{\rx \sim p_p}[\ell(\net(\rx), +1)]\;; \; R_n^-(g) = \E_{\rx \sim p_n}[\ell(\net(\rx), -1)]
\end{flalign}


==> assets/exp/tab_adni_dlrm.tex <==
\begin{table*}
\small 
\centering
\begin{tabular}{@{}cccccc@{}}
\toprule
Dataset
& PN         
& PvU 
& uPU
& nnPU
& ConPU
\\ \midrule\midrule
ADNI
&
&
& $73.45\textcolor{gray}{\pm 1.77}$
& $75.96\textcolor{gray}{\pm 1.42}$
&
\\\midrule 
Criteo-Kaggle
& $66.141$
& 
& 
& $74.52$
&
\end{tabular}
\caption{Results on ADNI and Criteo Kaggle Dataset ... }
\label{tab:adni.dlrm_exp}
\end{table*}


% \begin{table}
% \centering
% \begin{tabular}{@{}ccc@{}}
% \toprule
% Algorithm         & ADNI & Criteo-Kaggle \\ \midrule\midrule
% uPU~\citep{du2014analysis}              & $73.45\textcolor{gray}{\pm 1.77}$   &      \\
% nnPU~\citep{kiryo2017positive}          & $75.96\textcolor{gray}{\pm 1.42}$   &      \\
% % DAN               & 89.71   &      \\
% % VPU               &  -  &    89.5  \\
% SelfPU~\citep{chen2020self}             & $79.50\textcolor{gray}{\pm 1.80}$  &     \\
% ConPU {\bf (This work)}                 &    &      \\ \bottomrule
% \end{tabular}
% \caption{Results on ADNI and Criteo Kaggle Dataset ... }
% \label{tab:adni.dlrm_exp}
% \end{table}

==> assets/exp/tab_dataset_details.tex <==
\begin{table*}[htb!]
\small 
\centering
\begin{tabular}{@{}cccc@{}}
\toprule
%\footnotesize
Dataset & \#Train / \# Test & $\pi^\ast$ & Positive / Negative       \\ \midrule \midrule
MNIST   & 60k/10k & 0.49 & Odd / Even \\
CIFAR10 & 50k/10k & 0.40 & Vehicle/Animal\\
\bottomrule
\end{tabular}
\caption{Summary of datasets and optimal value of positive prior.}
\label{tab:datset}
\end{table*}


==> assets/exp/tab_mnist_PU.tex <==
\begin{table*}%[!htbp]
\small 
\centering
\begin{tabular}{@{}ccc@{}}
\toprule
Algorithm         & $n_P$ = 1k & $n_P$=3k \\ \midrule\midrule
uPU~\citep{du2014analysis}               & $92.52\textcolor{gray}{\pm 0.39}$  &      \\
nnPU~\citep{kiryo2017positive}              & $93.41\textcolor{gray}{\pm 0.20}$  &      \\
% DAN               & -   &      \\
% VPU               & -   &      \\
SelfPU~\cite{chen2020self}            & $94.21\textcolor{gray}{\pm 0.54}$  &     $96\textcolor{gray}{\pm 0.29}$ \\
ConPU {\bf (This work)} & {\bf 97.94}   &      \\ \bottomrule
\end{tabular}
\caption{Bin MNIST results ... }
\label{tab:mnist_exp}
\end{table*}

==> assets/introduction/assmp.scar.tex <==
\begin{assumption}[{\bf SCAR : Selected Completely At Random}]
\label{assm:selected_at_rand}
The labeled positive samples are sampled uniformly at random from all positive examples~\citep{elkan2008learning} 
% Formally speaking:
% \begin{flalign}
% \label{eq:SCAR}
% p(s=1 | \vx, y=1) = p(s=1 | y=1) = c
% \end{flalign}
% Intuitively, this simply means that, 
i.e. if the underlying true label is $y=1$ then the {\bf probability that a positive sample is labeled is constant} regardless of $\vx$ implying {\bf all the positive examples have the same probability of being labeled}.
% {\bf $s$ and $\vx$ are conditionally independent given $y$}. In other words it means that {\bf all the positive examples have the same probability of being labeled}. 
% Note that SCAR is equivalent to the missing completely at random assumption commonly made for learning from data with missing values~\citep{liu2003building, smith2007making}.
\end{assumption}

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
% %%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{section:conclusion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{See Section~\ref{section:conclusion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{All the code and models will be open sourced.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNA{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> figs/compare_CLR.tex <==
\begin{wrapfigure}{r}{0.4\textwidth}
% \vspace*{-2 em}
  \begin{center}
    \includegraphics[width=0.4\textwidth]{img/compare_pu_algos.png}
  \end{center}
 \caption{{\footnotesize {\bf Comparison of contrastive losses}: ResNet-18 trained on PU CIFAR (vehicle / animal) for varying number of labeled positive samples $n_P$ = 1k(2\%), 3k(6\%)}, 10k(20\%). The proposed contrastive loss {\bf puNCE} significantly improves over current.}
 \label{fig:compare_clr}
% \vspace*{-1 em}
\end{wrapfigure}

==> figs/datasets_plot.tex <==
\begin{figure}[]
\subfloat[\footnotesize{Supervised}]{\includegraphics[width=0.25\textwidth]{img/Dataset/sup_data.png}}
\subfloat[\footnotesize{Semi Supervised}]{\includegraphics[width=0.25\textwidth]{img/Dataset/semi_sup_data.png}}
\subfloat[\footnotesize{Positive Unlabeled}]{\includegraphics[width=0.25\textwidth]{img/Dataset/pu_data.png}}
\subfloat[\footnotesize{Unsupervised}]{\includegraphics[width=0.25\textwidth]{img/Dataset/unsup_data.png}}
\caption{\footnotesize }
\label{figure:data_setting}
\end{figure}
